Knowledge Graph Induction enabling Recommending and Trend Analysis: A Corporate Research Community Use Case

A research division plays an important role of driving innovation in an organization. Drawing insights, following trends, keeping abreast of new research, and formulating strategies are increasingly becoming more challenging for both researchers and executives as the amount of information grows in both velocity and volume. In this paper we present a use case of how a corporate research community, IBM Research, utilizes Semantic Web technologies to induce a unified Knowledge Graph from both structured and textual data obtained by integrating various applications used by the community related to research projects, academic papers, datasets, achievements and recognition. In order to make the Knowledge Graph more accessible to application developers, we identified a set of common patterns for exploiting the induced knowledge and exposed them as APIs. Those patterns were born out of user research which identified the most valuable use cases or user pain points to be alleviated. We outline two distinct scenarios: recommendation and analytics for business use. We will discuss these scenarios in detail and provide an empirical evaluation on entity recommendation specifically. The methodology used and the lessons learned from this work can be applied to other organizations facing similar challenges.

==> sections/evaluation.tex <==
\section{Entity Recommendation Evaluation}

\subsection{Experimental Design}
As previously mentioned we began by creating a proof of concept of a recommender engine based using the knowledge graph and our exploitation patterns as the foundation.  Initial anecdotal results were promising but the result set (less than 10) was too sparse to draw definitive conclusions.  We then put out a call to action for volunteers from various disciplines to participate in our study with the goal of having 30 or more participants.  

For each participant we used our new recommender service to generate 10 recommended projects, 10 recommended papers, and 5 achievements. Using these results we generated a unique survey for each participant and asked them to rate the recommendations on the following scale:

\begin{itemize}
    \item NONE: No value to me
    \item LOW: Good to know but I am not going to read anytime soon
    \item MEDIUM: Relevant for my specific area of interest (must read)
    \item HIGH: Relevant to my current project(s) and work
\end{itemize}

In addition we asked the users for an overall assessment of the service and, if possible, could they explain their reasoning. We were then able to collate the results on both a quantitative and qualitative scale.

We have analyzed the user feedback quantitatively using the Mean Average Precision (MAP) and Precision@K (P@K) metrics, that are metrics commonly adopted for evaluating recommendation systems. MAP measures the capability of the recommendation system to rank the relevant items at the top of the list. P@K is a set based metric by measuring the percentage of relevant items for the top-K items in the list.

Both MAP and P@K take in consideration only binary assessments, i.e. if the recommended item is relevant or non-relevant.
In order to convert our graded rating into a binary assessment, we adopt three different criteria, namely HIGH, MEDIUM, LOW, to differentiate which items to consider relevant from those non-relevant.
As shown in Table~\ref{tab:rec_results}, 


\begin{table}[t]
\centering
\bgroup
\setlength{\tabcolsep}{5pt}
\def\arraystretch{1.2}
\begin{tabular}{l|cc|cc|cc} 
\toprule
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\centering \textbf{Scholarly Articles}} & \multicolumn{2}{c|}{\centering \textbf{Projects}} & \multicolumn{2}{c}{\centering \textbf{Achievements}} \\ \hline
Criteria& MAP &P @ 10 & MAP & P @ 10 & MAP & P @ 5\\ \hline
\textbf{LOW+} & 0.89 & 0.76 & 0.92  & 0.81 & 0.87 & 0.82   \\
\textbf{MEDIUM+} &  0.51 & 0.34 & 0.65  & 0.45 & 0.51 & 0.36    \\
\textbf{HIGH} &  0.21 & 0.08 & 0.50  & 0.14 & 0.41 & 0.17  \\ 
\bottomrule
\end{tabular}
\egroup
\caption{User evaluation for scholary article, project and achievement recommendations for 30 users.}
\label{tab:rec_results}
\end{table}

We have also analyzed the reasons provided by the users to understand the main reasons for irrelevant recommendations. One repeating pattern was the users who have recently moved to a different research area or a project. Their historical profile of publication and previous projects didn't match their current expectations based on changes in research directions. As future work, we will explore how to detect such cases and adapt our recommendations. Furthermore, we also identified some cases where some relations between people, projects and publications that are not captured in our data models such as indirect collaborations and informal projects. In such cases, some of the recommended entities were obvious and known to the user (but not filtered because that information was not present in the KG).

==> sections/uptake.tex <==



\section{Uptake and Potential Impact}

This year, we intend to deploy the recommender technology to all users of the Apps@Research tools - on the order of 6,000 IBMers, using a phased approach. Our objectives:
\begin{itemize}
    \item Demonstrate usage of the technology by 20\% of active users.
    \item Demonstrate impact to accelerating innovation with 2 user / stakeholder testimonials about how app features catalyzed new research
    \item 1 testimonial from business development / client engagement stakeholders
    \item Increase frequency of use of applications 10\% (click rates, increase in monthly unique users who visited recommendations)
    \item Drive users to keep content up to date more often: recommender users to more frequently update projects / add progress reports / add papers 
    \item Improvements to Net Promoter Score / Customer Satisfaction score for the applications
    \item Continuous improvement of quality of recommendations as measured from user feedback
\end{itemize}

We envision both in-app and ``meet users where they are'' experiences outside the apps. In all cases, we will provide feedback mechanisms (e.g. thumbs up/down, free text explanations) for users to share their view on the quality of the recommendations. The intention is to feed this back into the machine learning model to learn and improve.

Initial UI / UX concepts include an email (see Figure~\ref{fig:ai_concept_one}) or slack subscription, wherein users would be recommended of paper, projects, accomplishments, data sets and / or subject matter experts, which would then link into the application for further perusal.

\begin{figure}[h!]
\includegraphics[width=\textwidth]{figures/ai-concept-one.png}
\caption{Example wireframes for recommended projects, people, or papers in various formats} \label{fig:ai_concept_one}
\end{figure}

\subsection{Extended Use Cases}

In addition to trend analysis, we believe KG technology could also be leveraged for flexible and on-demand business analytics, providing powerful insights to accelerate business, for example: (a) \textbf{Foresight:} What are the emerging trends in various research areas? (b)\textbf{Predicting success:} what are the characteristics of research projects that result in product revenue and other business impact, publications, recognitions and awards. How do we invest in new projects that exhibit these characteristics to better steer the IBM research agenda? Which papers should we support to have the best chance of publication at key conferences? (c) \textbf{Business development:} Quickly identifying relevant research activity of interest to current or prospective clients or partners (d) \textbf{Operations and efficiency:} Who is working on what projects and is time being used effectively? Is there duplicate activity? Where are the gaps? What are best opportunities for cross-collaboration?
(e) \textbf{Talent:} Who are the rising stars? How do we find the right projects for them, or nominate them for external awards? (f) \textbf{Portfolio:} Tracing research projects and outcomes to Objects and Key Results.


% \begin{itemize}
%     \item \textbf{Foresight:} What are the emerging trends in various research areas?
%     \item \textbf{Predicting success:} what are the characteristics of research projects that result in product revenue and other business impact, publications, recognitions and awards. How do we invest in new projects that exhibit these characteristics to better steer the IBM research agenda? Which papers should we support to have the best chance of publication at key conferences?
%     \item \textbf{Business development:} Quickly identifying relevant research activity of interest to current or prospective clients or partners
%     \item \textbf{Operations and efficiency:} Who is working on what projects and is time being used effectively? Is there duplicate activity? Where are the gaps? What are best opportunities for cross-collaboration?
%     \item \textbf{Talent:} Who are the rising stars? How do we find the right projects for them, or nominate them for external awards?
%     \item \textbf{Portfolio:} Tracing research projects and outcomes to Objects and Key Results
% \end{itemize}

\subsubsection{Commercialization of Research Assets}

Our philosophy is what we learn from this effort among the IBM Research community is a sandbox for a greater opportunity to accelerate discovery in the global scientific community. Knowledge induced and graphed from millions of documents could allow scientists around the world to more quickly discover relevant work, techniques, etc by others in similar or disparate fields and potential opportunities for collaboration. This can accelerate the pace of innovation in a world dominated by disconnected conference and journal publications and interpersonal networks.
